The dynamics of stars around spiral arms

Spiral density wave theory attempts to describe the spiral pattern in spiral galaxies in terms of a long-lived wave structure with a constant pattern speed in order to avoid the winding dilemma. The pattern is consequently a rigidly rotating, long-lived feature. We run N-body simulations of a giant disc galaxy consisting of a pure stellar disc and a static dark matter halo, and find that the spiral arms are transient features whose pattern speeds decrease with radius, in such a way that the pattern speed is almost equal to the rotation curve of the galaxy. We trace particle motion around the spiral arms. We show that particles from behind and in front of the spiral arm are drawn towards and join the arm. Particles move along the arm in the radial direction and we find a clear trend that they migrate toward the outer (inner) radii on the trailing (leading) side of the arm. Our simulations demonstrate that because the spiral arm feature is co-rotating, the particles continue to be accelerated (decelerated) by the spiral arm for long periods, which leads to strong and efficient migration, at all radii in the disc.

==> jour.tex <==

% 1998/08/12  Jonathan Baker 
% Renamed to mn-jour.bib.  Frequently cited journals for MNRAS have
% been modified to use the correct abbreviation, and some journals
% from the AASTeX macros have been added.

% $Log: mn-jour.bib,v $
% Revision 1.2  1998/08/30 22:35:46  jbaker
% Added RCS keywords.
%

% Copyright (C) 1990 Sake J. Hogeveen.

% This is MNEMONIC.BIB, a bibliography database file that provides mnemonics
% for journal names, which can be used in the `journal' field of bibliography
% entries in databases for BibTeX.
% The abbreviations of the journal names in this file follow the rules of
% the International List of Periodical Title Word Abbreviations.
% From: Astronomy and Astrophysics Abstracts, 1990, Vol. 49A

% Copyright Notice:
% The files ASTRON.BST, ASTRON.STY, ASTDOC.TEX, ASTDOC.BIB, EXAMPLE.TEX,
% EXAMPLE.BIB, MNEMONIC.BIB, and TEMPLATE.BIB are a package.
% You may copy and distribute them freely for non-commercial purposes,
% provided that you keep the package together and this copyright notice
% in tact.
% You may not alter or modify the files; this helps to ensure that all
% distributions of ASTRON.BST and related files are the same.
% If you make any modifications, then you must give the files new names,
% other than the present.
% The author bears no responsibilities for errors in this document or
% the software it describes; and shall not be held liable for any indirect,
% incidental, or consequential damages.

@STRING{aao = "AAO Newsl."}
@STRING{aavso = "AAVSO Newsl."}
@STRING{acta = "Acta Astron."}
@STRING{aaguv = "Acta Astron. Geophys. Univ. Comenianae"}
@STRING{actastsin = "Acta Astron. Sin."}
@STRING{actapsin = "Acta Astrophys. Sin."}
@STRING{agg = "Acta Geod. Geophys."}
@STRING{ags = "Acta Geophys. Sin."}
@STRING{appsb = "Acta Phys. Pol., Ser. B"}
@STRING{atash = "Acta Tech. Acad. Sci. Hung."}
@STRING{advp = "Adv. Phys."}
@STRING{advsr = "Adv. Space Res."}
@STRING{aip = "AIP Conf. Proc."}
@STRING{aavsob = "Am. Assoc. Variable Star Obs. Bull."}
@STRING{aavsoc = "Am. Assoc. Variable Star Obs. Circ."}
@STRING{amjp = "Am. J. Phys."}
@STRING{aatar = "Anglo--Aust. Telesc., Annu. Rep."}
@STRING{ag = "Ann. Geophys."}
@STRING{araa = "ARA\&A"} % "Ann. Rev. Astron. Astrophys."
@STRING{apl = "Ann. Phys. (Leipzig)"}
@STRING{apny = "Ann. Phys. (N.Y.)"}
@STRING{app = "Ann. Phys. (Paris)"}
@STRING{ao = "Appl. Opt."}
@STRING{appl = "Appl. Phys. Lett."}
@STRING{apb = "Appl. Phys., B"}
@STRING{as = "Appl. Spectrosc."}
@STRING{ahes = "Arch. Hist. Exact Sci."}
@STRING{archuk = "Archeoastronomy (U.K.)"}
@STRING{asbts = "Archenhold--Sternw. Berlin--Treptow, Sonderdr."}
@STRING{asbtvs = "Archenhold--Sternw. Berlin--Treptow, Vortr. Schr."}
@STRING{aonaicnl = "Arecibo Obs./NAIC, Newsl."}
@STRING{artsat = "Artif. Satell."}
@STRING{aiisao = "Astrofiz. Issled. Izv. Spets. Astrofiz. Obs."}
@STRING{af = "Afz"} % "Astrofizika"
@STRING{aa = "A\&A"} % "Astron. Astrophys."
@STRING{aar = "A\&AR"} % "Astron. Astrophys. Rev."
@STRING{aas = "A\&AS"} % "Astron. Astrophys. Suppl. Ser."
@STRING{abco = "Astron. Bull. (Carter Obs.)"}
@STRING{agas = "Astron. Ges., Abstr. Ser."}
@STRING{asther = "Astron. Her."}
@STRING{aiubc = "Astron. Inst. Univ. Brno, Contrib."}
@STRING{astj = "AJ"} % "Astron. J."
@STRING{an = "Astron. Nachr."}
@STRING{astnow = "Astron. Now"}
@STRING{astraum = "Astron. Raumfahrt"}
@STRING{astriha = "Astron. Rechen-Inst.Heidelb., Mitt., Ser. A"}
@STRING{astrihb = "Astron. Rechen-Inst.Heidelb., Mitt., Ser. B"}
@STRING{astschu = "Astron. Sch."}
@STRING{asttid = "Astron. Tidsskr."}
@STRING{asttsir = "Astron. Tsirk."}
@STRING{astvest = "Astron. Vestn."}
@STRING{astzh = "AZh"} % "Astron. Zh."
@STRING{astuai = "Astronomia UAI"}
@STRING{astie = "Astronomie"}
@STRING{asty = "Astronomy"}
@STRING{apj = "ApJ"} % "Astrophys. J."
@STRING{apjl = "ApJ"} % "Astrophys. J. Lett."
@STRING{apjss = "ApJS"} % "Astrophys. J. Suppl. Ser."
@STRING{aplc = "Astrophys. Lett. Commun."}
@STRING{apss = "Astrophys. Space. Sci."}
@STRING{apss = "Astrophys. Space. Sci."}
@STRING{ap = "Astrophysics"}
@STRING{aanlsor = "Atti Accad. Naz. Lincei, Ser. Ottava, Rend."}
@STRING{ajast = "Aust. J. Astron."}
@STRING{ajp = "Aust. J. Phys."}
@STRING{bavm = "BAV Mitt."}
@STRING{bavr = "BAV Rundbrief"}
@STRING{bbsag = "BBSAG Bull."}
@STRING{bestarnl = "Be Star Newsl."}
@STRING{bildw = "Bild Wiss."}
@STRING{bipm = "BIPM Circ. T"}
@STRING{boaumkt = "Biul. Obs. Astron. Uniw. M. Kopernika Toruniu"}
@STRING{boe = "Bol. Obs. Ebro"}
@STRING{broa = "Bol. ROA"}
@STRING{blm = "Boundary-Layer Meteorol."}
@STRING{boop = "Boyden Obs., Occas. Publ."}
@STRING{bastac = "Br. Astron. Assoc. Circ."}
@STRING{bjp = "Bulg. J. Phys."}
@STRING{baas = "BAAS"} % "Bull. Am. Astron. Soc."
@STRING{baps = "Bull. Am. Phys. Soc."}
@STRING{bafoev = "Bull. Assoc. Fr. Obs. Etoiles Variables"}
@STRING{bastic = "Bull. Astron. Inst. Czech."}
@STRING{basi = "Bull. Astron. Soc. India"}
@STRING{bain = "Bull. Astron. Inst. Netherlands"}
@STRING{bcao = "Bull. Crimean Astrophys. Obs."}
@STRING{bgsi = "Bull. Geogr. Surv. Inst."}
@STRING{bicds = "Bull. Inf. Cent. Donn\'ees Stellaires"}
@STRING{boab = "Bull. Obs. Astron. Belgr."}
@STRING{crassgvs = "C. R. Acad. Sci., S\'er. G\'en., Vie Sci."}
@STRING{crassii = "C. R. Acad. Sci., II"}
@STRING{cjp = "Can. J. Phys."}
@STRING{cm = "Celest. Mech."}
@STRING{cassos = "Cent. Astron. Sci. Spat., Obs. Sol."}
@STRING{cent = "Centaurus"}
@STRING{cpl = "Chem. Phys. Lett."}
@STRING{chinaa = "Chin. Astron. Astrophys."}
@STRING{chinp = "Chin. Phys."}
@STRING{chinpl = "Chin. Phys. Lett."}
@STRING{ciel = "Ciel"}
@STRING{cielt = "Ciel Terre"}
@STRING{ccotl = "Circ. Czech. Obs. Time Lattiude"}
@STRING{cinf = "Circ. Inf."}
@STRING{ctls = "Circ. Time Latitude Serv."}
@STRING{cqg = "Classical Quantum Gravity"}
@STRING{cast = "Comments Astrophys."}
@STRING{cnpp = "Comments Nucl. Part. Phys."}
@STRING{cppcf = "Comments Plasma Phys. Controlled Fusion"}
@STRING{cfsua = "Commun. Fac. Sci. Univ. Ankara, Ser. A2, A3"}
@STRING{cko = "Commun. Konkoly Obs."}
@STRING{cmp = "Commun. Math. Phys."}
@STRING{culo = "Commun. Univ. Lond. Obs."}
@STRING{comp = "Comput. Phys."}
@STRING{compcom = "Comput. Phys. Commun."}
@STRING{cp = "Contemp. Phys."}
@STRING{caosp = "Contrib. Astron. Obs. Skalnat\'e Pleso"}
@STRING{cap = "Contrib. Atmos. Phys."}
@STRING{cdaut = "Contrib. Dep. Astron., Univ. Tokyo"}
@STRING{clo = "Contrib. Lick Obs."}
@STRING{cncopb = "Contrib. Nicholas Copernicus Obs. Planetarium Brno"}
@STRING{cnjro = "Contrib. Nizamiah Japal-Rangapur Obs."}
@STRING{cpp = "Contrib. Plasma Phys."}
@STRING{cvvo = "Contrib. Van Vleck Obs."}
@STRING{cr = "Cosmic Res."}
@STRING{cryo = "Cryogenics"}
@STRING{czjp = "Czech. J. Phys., Sect. B"}
@STRING{drho = "Data Rep. Hydrogr. Obs., Ser. Astron. Geod."}
@STRING{dgkbawb = "Dtsch. Geod. Komm. Bayer. Akad. Wiss., Reihe B"}
@STRING{dgkbawc = "Dtsch. Geod. Komm. Bayer. Akad. Wiss., Reihe C"}
@STRING{dgkbawe = "Dtsch. Geod. Komm. Bayer. Akad. Wiss., Reihe E"}
@STRING{epsl = "Earth Planet. Sci. Lett."}
@STRING{erb = "Earth Rotation Bull."}
@STRING{emp = "Earth, Moon, Planets"}
@STRING{esrev = "Earth--Sci. Rev."}
@STRING{esab = "ESA Bull."}
@STRING{esaiuenl = "ESA IUE Newsl."}
@STRING{esaj = "ESA J."}
@STRING{esoar = "ESO Ann. Rep."}
@STRING{ejp = "Eur. J. Phys."}
@STRING{epl = "Europhys. Lett."}
@STRING{epn = "Europhys. News"}
@STRING{expast = "Exp. Astron."}
@STRING{fiz = "Fizika"}
@STRING{fortp = "Fortschr. Phys."}
@STRING{fp = "Found. Phys."}
@STRING{funcp = "Fundam. Cosmic Phys."}
@STRING{gaab = "G.~A.A.B."}
@STRING{gast = "G. Astron."}
@STRING{gem = "Gemini"}
@STRING{grg = "Gen. Relativ. Gravitation"}
@STRING{gca = "Geochim. Cosmochim. Acta"}
@STRING{ga = "Geomagn. Aehron."}
@STRING{gafd = "Geophys. Astrophys. Fluid Dyn."}
@STRING{gj = "Geophys. J."}
@STRING{grl = "Geophys. Res. Lett."}
@STRING{geo = "Geophysics"}
@STRING{geos = "GEOS Circ."}
@STRING{gbg = "Gerlands Beitr. Geophys."}
@STRING{heav = "Heavens"}
@STRING{hpa = "Helv. Phys. Acta"}
@STRING{hepnp = "High Energ. Phys. Nucl. Phys."}
@STRING{hob = "Hvar Obs. Bull."}
@STRING{hi = "Hyperfine Interact."}
@STRING{iappp = "I.A.P.P.P. Commun."}
@STRING{iauc = "IAU Circ."}
@STRING{iauib = "IAU Inf. Bull."}
@STRING{icarus = "Icarus"}
@STRING{i3etm = "IEEE Trans. Magn."}
@STRING{i3etns = "IEEE Trans. Nucl. Sci."}
@STRING{i3etps = "IEEE Trans. Plasma Sci."}
@STRING{iersbb = "IERS Bull. B"}
@STRING{iersba = "IERS Bull.--A"}
@STRING{ijpap = "Indian J. Pure Appl. Phys."}
@STRING{ijrsp = "Indian J. Radio Space Phys."}
@STRING{ibvs = "Inf. Bull. Variable Stars"}
@STRING{iaatub = "Inst. Astron. Astrophys. Tech. Univ. Berlin, Mitt."}
@STRING{iag = "Inst. Astron. Geod., Univ. Madr., Publ."}
@STRING{ia = "Inst. Astron., Univ. Camb., Annu. Rep."}
@STRING{icq = "Int. Comet Q."}
@STRING{ijimw = "Int. J. Infrared Millimeter Waves"}
@STRING{ijmp = "Int. J. Mod. Phys. A"}
@STRING{ijtp = "Int. J. Theor. Phys."}
@STRING{ip = "Inverse Probl."}
@STRING{iastj = "Ir. Astron. J."}
@STRING{iris = "IRIS Bull. A"}
@STRING{iskz = "Issled. Solntsa Krasnykh Zvezd"}
@STRING{intsa = "Itogi Nauki Tekh., Ser. Astron."}
@STRING{intsppk = "Itogi NAuki Tekh., Ser. Plazmennye Protsessy Kosmose"}
@STRING{iaoe = "Izv. Astron. Obs. Ehngel'gardt."}
@STRING{ikao = "Izv. Krym. Astrofiz. Obs."}
@STRING{ivuzr = "Izv. Vyssch. Uchebn. Zaved., Radiofiz."}
@STRING{jasa = "J. Acoust. Soc. Am."}
@STRING{jaavso = "J. Am. Assoc. Variable Star Obs."}
@STRING{jam = "J. Appl. Meteorol."}
@STRING{jap = "J. Appl. Phys."}
@STRING{jastf = "J. Astron. Fr."}
@STRING{japast = "JA\&A"} % "J. Astrophys. Astron."
@STRING{jas = "J. Atmos. Sci."}
@STRING{jatp = "J. Atmos. Terr. Phys."}
@STRING{jbasta = "J. Br. Astron. Assoc."}
@STRING{jbis = "J. Br. Interplanet. Soc."}
@STRING{jcp = "J. Chem. Phys."}
@STRING{jcomp = "J. Comp. Phys."}
@STRING{jel = "J. Electrostat."}
@STRING{jfseu = "J. Fac Sci., Ege Univ., Ser. A"}
@STRING{jfm = "J. Fluid Mech."}
@STRING{jgr = "J. Geophys. Res."}
@STRING{jhast = "J. Hist. Astron."}
@STRING{jms = "J. Mater. Sci."}
@STRING{jmp = "J. Math. Phys."}
@STRING{jmo = "J. Mod. Opt."}
@STRING{jop = "J. Opt. (Paris)"}
@STRING{josaa = "J. Opt. Soc. Am. A"}
@STRING{josab = "J. Opt. Soc. Am. B"}
@STRING{jp = "J. Phys."}
@STRING{jpa = "J. Phys. A"}
@STRING{jpb = "J. Phys. B"}
@STRING{jpd = "J. Phys. D"}
@STRING{jpe = "J. Phys. E"}
@STRING{jpg = "J. Phys. G"}
@STRING{jpsj = "J. Phys. Soc. Jpn."}
@STRING{jpp = "J. Plasma Phys."}
@STRING{jqsrt = "J. Quant. Spectrosc. Radiat. Transfer"}
@STRING{jrasc = "J. R. Astron. Soc. Can."}
@STRING{jsp = "J. Stat. Phys."}
@STRING{jvst = "J. Vac. Sci. Technol., A"}
@STRING{jetpl = "JETP Lett."}
@STRING{jhatd = "Johns Hopkins APL Tech. Dig."}
@STRING{jjap1 = "Jpn. J. Appl. Phys., Part 1"}
@STRING{jjap2 = "Jpn. J. Appl. Phys., Part 2"}
@STRING{kai = "Kapteyn Astron. Inst., Annu. Rep."}
@STRING{kexto = "Kexue Tongbao"}
@STRING{kfnt = "Kinematika Fiz. Nebesn. Tel"}
@STRING{kob = "Kodaikanal Obs. Bull."}
@STRING{kt = "Komet. Tsirk."}
@STRING{ki = "Kosm. Issled."}
@STRING{koz = "Kozmos"}
@STRING{kpm = "KPM"}
@STRING{lo = "Laser Optoelektron."}
@STRING{latc = "Latitude Circ."}
@STRING{lest = "LEST Found., Annu. Rep."}
@STRING{lmp = "Lett. Math. Phys."}
@STRING{lob = "Lick Obs. Bull."}
@STRING{mg = "Manuscr. Geod."}
@STRING{ml = "Mater. Lett."}
@STRING{mrb = "Mater. Res. Bull."}
@STRING{mfs = "Mem. Fac. Sci., Kyoto Univ., Ser. Phys., Astrophys., Geophys., Chem."}
@STRING{memras = "Mem. R. Astron. Soc."}
@STRING{msai = "Mem. Soc. Astron. Ital."}
@STRING{merc = "Mercury"}
@STRING{mess = "Messenger"}
@STRING{met = "Meteoritics"}
@STRING{metka = "Meteoritika"}
@STRING{metro = "Metrologica"}
@STRING{mpb = "Minor Planet Bull."}
@STRING{mpc = "Minor Planet Circ."}
@STRING{masbt = "Mitt. Archenold--Sternw. Berlin Treptow"}
@STRING{mag = "Mitt. Astron. Ges."}
@STRING{mlotud = "Mitt. Lohrmann--Obs., Tech. Univ. Dresden"}
@STRING{mss = "Mitt. Sternw. Sonneberg"}
@STRING{mvs = "Mitt. Ver{\"a}nderliche Sterne"}
@STRING{mzpe = "Mitt. Zentralinst. Phys. Erde"}
@STRING{mpla = "Mod. Phys. Lett. A"}
@STRING{mn = "MNRAS"} % "Mon. Not. R. Astron. Soc."
@STRING{mnassa = "Mon. Notes Astron. Soc. S. Afr."}
@STRING{nint = "Nablyud. Iskusstv. Nebesn. Tel."}
@STRING{nogb = "Nachr. Olbers--Ges. Bremen"}
@STRING{naoj = "Natl. Astron. Obs. (Jpn.), Repr."}
@STRING{ng = "Natl. Geogr."}
@STRING{nraoa = "Natl. Radio Astron. Obs., Repr., Ser. A"}
@STRING{nraob = "Natl. Radio Astron. Obs., Repr., Ser. B"}
@STRING{nat = "Nat"} % "Nature"
@STRING{natwis = "Naturwissenschaften"}
@STRING{ni = "Nauchn. Inf."}
@STRING{nlasny = "News Lett. Astron. Soc. N.Y."}
@STRING{nrodaour = "Nizamiah Rangapur Obs. Dep. Astron., Osmania Univ., Repr."}
@STRING{nraow = "NRAO Workshop"}
@STRING{nimpra = "Nucl. Instrum. Methods Phys. Res., Sect. A"}
@STRING{nimprb = "Nucl. Instrum. Methods Phys. Res., Sect. B"}
@STRING{npa = "Nucl. Phys. A"}
@STRING{npb = "Nucl. Phys. B, Part. Phys."}
@STRING{nca = "Nuovo Cimento A"}
@STRING{ncb = "Nuovo Cimento B"}
@STRING{ncc = "Nuovo Cimento C"}
@STRING{ot = "Obs. Trav."}
@STRING{obs = "Observatory"}
@STRING{onl = "Occultation Newsl."}
@STRING{ozvp = "{\"O}sterr. Z. Vermessungswes. Photogramm."}
@STRING{oc = "Opt. Commun."}
@STRING{oe = "Opt. Eng."}
@STRING{olt = "Opt. Laser Technol."}
@STRING{ol = "Opt. Lett."}
@STRING{on = "Opt. News"}
@STRING{os = "Opt. Spectrosc."}
@STRING{optik = "Optik"}
@STRING{ofeb = "Origins Life Evol. Biosphere"}
@STRING{orion = "Orion"}
@STRING{orione = "Orione"}
@STRING{oac = "Oss. Astrofis. Catania, Pubbl."}
@STRING{pz = "Perem. Zvezdy"}
@STRING{pb = "Phys. Bl."}
@STRING{pcm = "Phys. Chem. Miner."}
@STRING{pfa = "Phys. Fluids, A"}
@STRING{pfb = "Phys. Fluids, B"}
@STRING{pla = "Phys. Lett. A"}
@STRING{plb = "Phys. Lett. B"}
@STRING{pr = "Phys. Rep."}
@STRING{pra = "Phys. Rev. A"}
@STRING{prb = "Phys. Rev. B"}
@STRING{prc = "Phys. Rev. C"}
@STRING{prd = "Phys. Rev. D"}
@STRING{prl = "Phys. Rev. Lett."}
@STRING{ps = "Phys. Scr."}
@STRING{ptch = "Phys. Teach."}
@STRING{ptod = "Phys. Today"}
@STRING{pha = "Physica A"}
@STRING{phb = "Physica B"}
@STRING{phd = "Physica D"}
@STRING{paz = "Pis'ma Astron. Zh."}
@STRING{pss = "Planet. Space Sci."}
@STRING{ppcf = "Plasma Phys. Controlled Fusion"}
@STRING{pa = "Postepy Astron."}
@STRING{pram = "Pram\~{a}na"}
@STRING{pri = "Priroda"}
@STRING{pasa = "Proc. Astron. Soc. Aust."}
@STRING{pi3e = "Proc. IEEE"}
@STRING{prsl = "Proc. R. Soc. London, Ser. A"}
@STRING{posp = "Proceedings of SPIE"}
@STRING{past = "Prog. Astron."}
@STRING{ptp = "Prog. Theor. Phys."}
@STRING{paicas = "Publ. Astron. Inst. Czech. Acad. Sci."}
@STRING{pasj = "PASJ"} % "Publ. Astron. Soc. Jpn."
@STRING{pasp = "PASP"} % "Publ. Astron. Soc. Pac."
@STRING{pbao = "Publ. Beijing Astron. Obs."}
@STRING{pdaub = "Publ. Dep. Astron., Univ. Beogr."}
@STRING{pdao = "Publ. Dom. Astrophys. Obs."}
@STRING{pnlaoj = "Publ. Natl. Astron. Obs. Jpn."}
@STRING{ppmo = "Publ. Purple Mt. Obs."}
@STRING{psao = "Publ. Shaanxi Astron. Obs."}
@STRING{pscds = "Publ. Sp\'ec. Cent. Donn\'ees Stellaires"}
@STRING{pyo = "Publ. Yunnan Obs."}
@STRING{pag = "Pure Appl. Geophys."}
@STRING{qbsa = "Q. Bull. Sol. Act."}
@STRING{qjras = "QJRAS"} % "Q. J. R. Astron. Soc."
@STRING{rad = "Radiant"}
@STRING{rsci = "Radio Sci."}
@STRING{reche = "Recherche"}
@STRING{rpp = "Rep. Prog. Phys."}
@STRING{ra = "Rev. Astron."}
@STRING{rg = "Rev. Geophys."}
@STRING{rmf = "Rev. Mex. Fis."}
@STRING{rmp = "Rev. Mod. Phys."}
@STRING{rrp = "Rev. Roum. Phys."}
@STRING{rsi = "Rev. Sci. Instrum."}
@STRING{rnc = "Riv. Nuovo Cimento"}
@STRING{rh = "\v{R}\'{\i}\v{s}e hv\v{e}zd"}
@STRING{saaoar = "S. Afr. Astron. Obs., Annu. Rep."}
@STRING{saaoc = "S. Afr. Astron. Obs., Circ."}
@STRING{saaon = "SAAO Newsl."}
@STRING{sciam = "Sci. Am."}
@STRING{scch = "Sci. China, Ser. A"}
@STRING{srtu = "Sci. Rep. T\^{o}hoku Univ., Eighth Ser."}
@STRING{sc = "Sci"} % "Science"
@STRING{sar = "Sendai Astron. Rap."}
@STRING{st = "Sidereal Times"}
@STRING{sky = "Sky Telesc."}
@STRING{sbaavso = "Sol. Bull. (AAVSO)"}
@STRING{se = "Sol. Energy"}
@STRING{sp = "Sol. Phys."}
@STRING{srd = "Sol. Radio Data"}
@STRING{ssres = "Sol. Syst. Res."}
@STRING{sdb = "Soln. Dannye, Byull."}
@STRING{sonne = "Sonne"}
@STRING{sbo = "Soobshch. Byurak. Obs."}
@STRING{ssao = "Soobshch. Spets. Astrofiz. Obs."}
@STRING{sost = "South. Stars"}
@STRING{sa = "SvA"} % "Sov. Astron."
@STRING{sal = "SvA"} % "Sov. Astron. Lett."
@STRING{sjot = "Sov. J. Opt. Technol."}
@STRING{spd = "Sov. Phys. -- Dokl."}
@STRING{spj = "Sov. Phys. -- JETP"}
@STRING{spu = "Sov. Phys. -- Usp."}
@STRING{space = "Space"}
@STRING{ssr = "Space Sci. Rev."}
@STRING{stsi = "Space Telesc. Sci. Inst., Newsl."}
@STRING{sf = "Spaceflight"}
@STRING{sterne = "Sterne"}
@STRING{sw = "Sterne Weltraum"}
@STRING{sb = "Sternenbote"}
@STRING{strlast = "Strolling Astron."}
@STRING{sgg = "Stud. Geophys. Geod."}
@STRING{taot = "Tartu Astrof{\"u}{\"u}s. Obs. Teated"}
@STRING{tect = "Tectonophysics"}
@STRING{tellus = "Tellus, Ser. A"}
@STRING{tmf = "Teor. Mat. Fiz."}
@STRING{tp = "Theor. Pap."}
@STRING{tsb = "Time Serv. Bull."}
@STRING{tmnr = "Tokyo Meteor Network Rep."}
@STRING{tai = "Tsirk. Astron. Inst. (Tashkent)"}
@STRING{ufz = "Ukr. Fiz. Zh."}
@STRING{ucla = "Universe Classroom"}
@STRING{uao = "Upps. Astron. Obs., Rep."}
@STRING{urania = "Urania"}
@STRING{usnoc = "U.S. Nav. Obs., Circ."}
@STRING{usnos4 = "U.S. Nav. Obs., Ser. 4"}
@STRING{ufn = "Usp. Fiz. Nauk"}
@STRING{vsb = "Variable Star Bull."}
@STRING{vasiona = "Vasiona"}
@STRING{varih = "Ver{\"o}ff. Astron. Rechen--Inst. Heidelb."}
@STRING{vzpe = "Ver{\"o}ff. Zentralinst. Phys. Erde"}
@STRING{vesmir = "Vesm\'{\i}r"}
@STRING{vansssr = "Vestn. Akad. Nauk SSSR"}
@STRING{vku = "Vestn. Kiev. Univ., Astron."}
@STRING{va = "Vistas Astron."}
@STRING{wgn = "WGN"}
@STRING{wztud = "Wiss. Z. Tech. Univ. Dresden"}
@STRING{yama = "Yamamoto Circ."}
@STRING{zap = "Z. Astrophys."}
@STRING{zamp = "Z. Angew. Math. Phys."}
@STRING{zna = "Z. Naturforsch., A"}
@STRING{zpa = "Z. Phys., A"}
@STRING{zpc = "Z. Phys., C"}
@STRING{zv = "Zemlya Vselennaya"}
@STRING{zenit = "Zenit"}
@STRING{zetf = "Zh. Ehksp. Teor. Fiz."}


